Beyond Demographic Parity: Redefining Equal Treatment

Liberalism-oriented political philosophy reasons that all individuals should be treated equally independently of their protected characteristics. Related work in machine learning has translated the concept of \emph{equal treatment} into terms of \emph{equal outcome} and measured it as \emph{demographic parity} (also called \emph{statistical parity}). Our analysis reveals that the two concepts of equal outcome and equal treatment diverge; therefore, demographic parity does not faithfully represent the notion of \emph{equal treatment}. We propose a new formalization for equal treatment by (i) considering the influence of feature values on predictions, such as computed by Shapley values decomposing predictions across its features, (ii) defining distributions of explanations, and (iii) comparing explanation distributions between populations with different protected characteristics. We show the theoretical properties of our notion of equal treatment and devise a classifier two-sample test based on the AUC of an equal treatment inspector. We study our formalization of equal treatment on synthetic and natural data. We release \texttt{explanationspace}, an open-source Python package with methods and tutorials.

==> content/checklist.tex <==
\section*{Checklist}


%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerTODO{}
  \item Did you describe the limitations of your work?
    \answerYes{The work is limited to tabular datasets.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerTODO{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerTODO{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerTODO{}
        \item Did you include complete proofs of all theoretical results?
    \answerTODO{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{See reproducibility section}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{Yes, we don't do hyperparameter tunning, we use the default ones given by the packages.}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{Standard deviation is reported in the tables}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See reproducibility sectio}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{Scikit Learn, SHAP, Xgboost, Folkstables}
  \item Did you mention the license of the assets?
    \answerNo{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{Methods, code and experiments}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{We have used Folktables \cite{ding2021retiring} that provides code to download data from the American Community Survey (ACS) Public Use Microdata Sample (PUMS) files managed by the US Census Bureau. The data itself is governed by the terms of use provided by the Census Bureau.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}
\end{enumerate}


==> content/miscellaneous.tex <==
Even if deployed with the best intentions, machine learning methods can perpetuate, amplify or even create social biases. Measures of
(un-)fairness have been proposed as a way to gauge the (non-)discriminatory nature of machine learning models. 
However, proxies of protected attributes causing discriminatory effects remain challenging to address. In this work, we propose a  new algorithmic approach that measures group-wise demographic parity violations and allows us to inspect the causes of inter-group discrimination. Our method relies on the novel idea of measuring the dependence of a model on the protected attribute based on the explanation space, an informative space that allows for more sensitive audits than the primary space of input data or prediction distributions, and allowing for the assertion of theoretical demographic parity auditing guarantees. We provide  a mathematical analysis, synthetic examples, and experimental evaluation of real-world data. We release \texttt{nobias} an opensource Python package with methods, routines, and tutorials.

\section{Introduction}
%%%%%%% have a look at this %%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\url{https://www.youtube.com/watch?v=kyWyp-d0r94&ab_channel=TheConferenceonFairness%2CAccountability%2CandTransparency%28FAT%2a%29}
%https://www.linkedin.com/posts/ieaitum_ieai-2022-research-brief-ai-auditing-activity-6963460881514954752-snzA?utm_source=linkedin_share&utm_medium=android_app
% Intro to fairness and bias
\begin{figure}[ht]
    \centering
    \includegraphics[width=\columnwidth]{images/DPI.drawio.pdf}
    \caption{Demographic Parity Inspector($g_\psi$) workflow. The training of models is shaded in red while the derivations of explanations  are shaded in blue. The  model $f_\theta$ is learned based on training data, $\{(x_i,y_i)\}$,  and outputs the explanations $\Ss(f_\theta,X)$. The \enquote{DP Inspector} receives the explanations to predict the protected attribute, $Z$. Then if the AUC is above $0.5$ then there is a demographic parity violation. We can interpret the reasons for demographic parity violations on $g_\psi$ with explainable AI techniques}
    \label{fig:workflow}
\end{figure}


% What is the problem?

Notions of fair ML are ultimately based on redistributive justice and political philosophy frameworks. Then, those notions are interpreted by researchers and practitioners until they reach technical formulation that we can quantify in ML systems, by doing this reification of the entity often the metric divergers to the original notion.

%~\cite{rawls1958justice,rawls1991justice,rawls2020theory,arneson1989equality,dworkin1981equality,dworkin1981equality2}

In this paper, we focus on the notion of \enquote{equality of treatment}, a key concept in political philosophy that is often translated to the ML literature as \textit{statistical parity} or \enquote{demographic parity}.

The notion of \enquote{equality of treatment} implies that all individuals should be treated equally regardless of their protected characteristics. We identify this  notion as if the behaviour of a model $f$ is independent of a protected attribute $Z$, formally $f \perp Z$. 


This notion has been translated to Fair ML as \enquote{demographic or statistical parity}, which is often measured in the literature as  if the distributions of the predictions of a model $f(X)$ are equal between protected groups $d(P(f(X)|Z)=d(P(f(X)|Z)$.


There exists a range of metrics (demographic parity, equal opportunity, average absolute odds \ldots) that judge the \emph{global} degree of unfairness arising from the use of machine learning models. Together with some predictive performance measures (accuracy, precision, AUC \ldots), these metrics are commonly used to deliver classifiers that achieve high degrees of predictive performance and fairness e.g.\ \cite{zafat2017fairnessDisparate,negligible2021}.
% Why is it interesting??
Unfortunately,  approaches that enforce low measures of unfairness at the global level may cause new kinds of unfairness \emph{at the subgroup level}. As \cite{ruggieri23}
shows, pushing for well-balanced fairness among groups at such a global scale may imply novel discrimination at
inter-group levels leading to new kinds of unfairness introduced by an erroneous use of fair-AI methods. 

% Why is it hard?
The Yule’s effect~\cite{yule1900vii,simpson1951interpretation,pearson1899vi} occurs when positive and negative associations between the model predictions $f(X)$ and the protected attribute $Z$ cancel out producing a vanishing correlation in the mixture of the distribution. It occurs whenever we aim at group fairness, such as independence $f(X)\perp Z$, but we wrongly disregard control for the protected attribute $Z$. Fair machine learning algorithms may result in disparate effects on separate distributions, with some subgroups impacted positively (higher fairness) and other subgroups impacted negatively (lower fairness) \cite{ruggieri23}.
For example, enforcing fairness for one discriminated ethnic group at the country level may imply novel kinds of unfairness for the subgroup of this ethnicity in a particular local state.


% Pitfall of previous work 
Previous methods of measuring demographic parity have relied on the predictions in the output space whose low dimensionality is prone to fall under Yule's effect, and on statistical measures on input data that is model-independent. Furthermore, on many occasions detecting and quantifying fairness violations is not enough, there is also the need to pinpoint  \textit{What are the specific sources of discrimination?}. 

% What do we do
We address this problem by providing a novel kind of demographic parity measurement that analyzes how different protected groups are treated at the distributional and instance level and how each feature contributes to the demographic parity violation. This approach relies on the explanation space, a novel data space that has theoretical guarantees while performing demographic parity inspections.  Our main contributions are:
\begin{itemize}
    \setlength\itemsep{0.1em}

    \item We use the explanation space to measure fairness by providing theoretical guarantees and experiments with synthetic data and real data use cases.% The explanation space is more sensitive and indicative than input or prediction data spaces.

    %\item We overcome the Yule–Simpson's effect of demographic parity measurements on the predictions space.\carlos{I have no clue}
    
    \item We introduce a \enquote{Demographic Parity Inspector} method that allows for interpretable fairness quantification that sheds insights on the root causes of unfairness.

    \item We release an open-source Python package \texttt{nobias}, which implements our \enquote{Demographic Parity Inspector} that is \texttt{scikit-learn} compatible~\cite{pedregosa2011scikit}, together with code and tutorials for reproducibility.
    
\end{itemize}



==> notes/math_notes.tex <==
\newpage
\section{Notes on Math}
\todo[inline]{Remove the notes before submitting}
There are two ways to formalize the math of your experiments and you need to decide for one
\subsection{The Random Variables Way}
This way models the random variables and each sample is a realization of these.
This approach focuses on more on the theoretical model behind the experiments.

\paragraph{Basic Notion.}
Each random variable is given by an upper case character and might contain an additional distribution name, e.g. $X^{ood} \sim  N(0,\begin{bmatrix}1 & c \\c & 1 \end{bmatrix})$ \todo{I suggest to keep the distribution name always as upper index instead of mixing upper and lower position}.

Different feature dimensions are written as lower index, e.g. $X=(X_1,X_2)$ or 
\[X^{ood}=(X^{ood}_1,X^{ood}_2) \sim  N(0,\begin{bmatrix}1 & c \\c & 1 \end{bmatrix})\]

Consequently, the target variable would be defined as: $Y=X_1\cdot X_2 + \epsilon$ with $\epsilon \sim N(0,0.1)$.

An equivalent notion would be $Y\sim N(X_1\cdot X_2, 0.1)$

\paragraph{Samples and Sample Size.}
For the experiments (especially with statistical tests), it is important to know the sample size. Just use sentences like \emph{For the experiment, we draw 1000 realizations/samples of $X$ and 500 realizations of $X^{ood}$}.

If you need a concrete sample (in many cases you can just use the random variable), use lower case characters and a sentence like: \emph{Let $x=(x_1,x_2)$ be a realization of $X$, ...} \todo{DO NOT write something like $x\in X$}


\subsection{The Data-Centeres Way}
This way models the concrete data and is much closer to the concrete implementation.

\paragraph{Basic Notion.}
Matrices are written as upper case characters and vectors as lower case characters. Again, the name should always be at the same position (suggestion:upper index).
The connection between data and distribution is given in textual form:
\emph{$X=(x_1,x_2)$ is a $n\times 2$ matrix of $n=1000$ samples drawn from $N(0,\begin{bmatrix}1 & c \\c & 1 \end{bmatrix})$}\todo{DO NOT use $\in$ or $\sim$. Curve brackets $\{\ldots\}$ indicate sets. I would not use them.}
